End-to-end Speech Translation via Cross-modal Progressive Training

End-to-end speech translation models have become a new trend in research due to their potential of reducing error propagation. However, these models still suffer from the challenge of data scarcity. How to effectively use unlabeled or other parallel corpora from machine translation is promising but still an open problem. In this paper, we propose Cross Speech-Text Network (XSTNet), an end-to-end model for speech-to-text translation. XSTNet takes both speech and text as input and outputs both transcription and translation text. The model benefits from its three key design aspects: a self-supervised pre-trained sub-network as the audio encoder, a multi-task training objective to exploit additional parallel bilingual text, and a progressive training procedure. We evaluate the performance of XSTNet and baselines on the MuST-C En-X and LibriSpeech En-Fr datasets. In particular, XSTNet achieves state-of-the-art results on all language directions with an average BLEU of 28.8, outperforming the previous best method by 3.2 BLEU. Code, models, cases, and more detailed analysis are available at https://github.com/ReneeYe/XSTNet.

==> 00_data.tex <==

\begin{table}[h]
    \setlength{\abovecaptionskip}{-0.3cm}
    \setlength{\belowcaptionskip}{-0.cm}
    \centering
    \small
    \begin{tabular}{c|cr||cr}
        \toprule
         & \multicolumn{2}{c||}{\textbf{ST (MuST-C)}} & \multicolumn{2}{c}{\textbf{MT}} \\
         \textbf{En$\rightarrow$} & hours & \#sents & name & \#sents \\
        \hline
         \textbf{De} & 408 & 234K & WMT16 & 4.6M \\
         \textbf{Fr} & 492 & 292K & WMT14 & 40.8M \\
         \textbf{Ru} & 489 & 270K & WMT16 & 2.5M \\
        \bottomrule
    \end{tabular}
    \caption{Statistics of all datasets}
    \label{tab:data}
\end{table}

==> 01_vs_baselines.tex <==
\begin{table*}[!th]
    \setlength{\abovecaptionskip}{-0.3cm}
    \setlength{\belowcaptionskip}{-0.cm}
    \centering
    \small
    \begin{tabular}{l|c|c||cccc}
        \toprule
        \textbf{Models} & \textbf{External data} & \textbf{Pre-train tasks} &
        \textbf{En-De} & \textbf{En-Fr} & \textbf{En-Ru} & \textbf{Avg.} \\
        \midrule
        
        % BiLSTM~\cite{di2019must} & \texttimes & \texttimes & 
        %     12.9 & 22.3 & 7.22 & 14.1 \\
        % wav2vec+BiLSTM & \texttimes & \texttimes &
        %     - & 29.8 & - & -  \\
        % VGGTLarge & LL & ASR, MT &
        %     25.2 & - & - & - \\
        Transformer ST~\cite{zhao2020neurst}& \texttimes & ASR &
            22.8 & 33.3 & 15.1 & 23.7 \\
        % Cascade(Espnet) & \texttimes & \texttimes &
        %   23.6 & 33.8 &  16.4 &  24.6 \\
        % Cascade~\cite{zhao2020neurst} & \texttimes & \texttimes &
            % 23.4 & 33.9 &  16.0 &  24.4 (+0.7) \\
        % \hline
        
        AFS~\cite{zhang2020adaptive} & \texttimes & \texttimes & 
            22.4 & 31.6 & 14.7 & 22.9 (-0.8) \\
        Dual-Decoder Transf.~\cite{le2020dual} & \texttimes & \texttimes &
            23.6 & 33.5 & 15.2 & 24.1 (+0.4) \\
        STAST~\cite{liu2020bridging} & \texttimes & \texttimes &
            23.1 & - & - & - \\
        
        Tang et al.~\cite{tang2020general}  & MT & ASR, MT & 
            24.8 & 36.4 & - & -\\
        
        FAT-ST (Big)~\cite{zheng2021fused} & ASR, MT, mono-data$^\dagger$ & FAT-MLM &
            25.5 & - & - & - \\
            
        % \multirow{2}*{FAT-ST (big)} & ASR, audio-only & \multirow{2}*{MLM} & 
        %     \multirow{2}*{25.5} & - & - & - \\
        %  & MT, text-only & & & \\
        % \hline
        \midrule
        W-Transf. & audio-only* & SSL* & 
            23.6 & 34.6 & 14.4 & 24.2 (+0.5)\\
        % Wav2vec2+transformer (chi-fair) & \texttimes & 22.3 & 33.3 & 15.8 & \\
        % \hline
        % Strong-cascade & MT & \texttimes &
            % 25.2 & 34.9 & 17.0 & 25.7 (+2.0)\\
        \textbf{\method-Base} & audio-only* & SSL* & 
            25.5 & 36.0 & 16.9 & 26.1 (+2.4)\\
        \textbf{\method-Expand} & MT, audio-only* & SSL*, MT &
            \textbf{27.8} & \textbf{38.0} & \textbf{18.4} & \textbf{27.8 (+4.1)} \\
        
        \bottomrule
    \end{tabular}
    \caption{Performance (BLEU) on MuST-C En-De, En-Fr and En-Ru test sets. 
    $^\dagger$: ``Mono-data" means audio-only data from Librispeech, Libri-Light, as well as text-only data from Europarl/Wiki Text; 
    *: ``Audio-only" data from Librispeech audio data is used in the pre-training of wav2vec2.0-base module, and ``SSL" means the self-supervised learning from unlabeled audio data.}
    \label{tab:vs_baseline}
\end{table*}


